Residential Demand Response Targeting Using Machine Learning with Observational Data

The large scale deployment of Advanced Metering Infrastructure among residential energy customers has served as a boon for energy systems research relying on granular consumption data. Residential Demand Response aims to utilize the flexibility of consumers to reduce their energy usage during times when the grid is strained. Suitable incentive mechanisms to encourage customers to deviate from their usual behavior have to be implemented to correctly control the bids into the wholesale electricity market as a Demand Response provider. In this paper, we present a framework for short term load forecasting on an individual user level, and relate nonexperimental estimates of Demand Response efficacy, i.e. the estimated reduction of consumption during Demand Response events, to the variability of user consumption. We apply our framework on a data set from a residential Demand Response program in the Western United States. Our results suggest that users with more variable consumption patterns are more likely to reduce their consumption compared to users with a more regular consumption behavior.

==> sections/Acknowledgment.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% This is Acknowledgment.tex (part of Targeting.tex)
% author: Datong Zhou
% last edited: Feb 04, 2016
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% !TEX root = ../Targeting.tex

\section*{Acknowledgment}
\label{sec:Acknowledgment}
We thank Ohmconnect for providing us with the consumption data that enabled us to analyze residential Demand Response issues. In particular, we thank Matt Duesterberg (CEO of Ohmconnect), John Anderson, and Curtis Tongue for interesting discussions and the permission to utilize anonymized data for scientific analyses.

==> sections/Hypothesis_Test.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% This is Estimated_Treatment_Effects.tex (part of Targeting.tex)
% author: Datong Zhou
% last edited: Jan 07, 2016
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% !TEX root = ../Targeting.tex

\section{Estimated Treatment Effects of DR}
\label{sec:Estimated_Treatment_Effects_DR}
We now compare the samples $Y_i^1$ and $\hat{Y}_i^1$ with a nonparametric hypothesis test, whose goal is to determine that these samples stem from different distributions, that is, the null hypothesis states that both samples are generated by the same (unknown) distribution $F(u)$:
\begin{equation}\label{eq:null_hypothesis_samples}
H_0: Y_i^1, \hat{Y}_i^1 \sim F(u) \Longleftrightarrow Y_i^1 - \hat{Y}_i^1 = 0.
\end{equation}
We would like to falsify \eqref{eq:null_hypothesis_samples} and assume the validity of the one-sided alternative hypothesis $H_1$, namely that there is a notable difference in the distribution between $Y_i^1$ and $\hat{Y}_i^1$:
\begin{equation}\label{eq:alternative_hypothesis}
H_1: Y_i^1 \sim F(u),~ \hat{Y}_i^1 \sim F(u) + \Delta \Longleftrightarrow \hat{Y}_i^1 - Y_i^1 = \Delta.
\end{equation}
In \eqref{eq:alternative_hypothesis}, it is assumed that the predicted outcomes $\hat{Y}_i^1$ are generated by the same (unknown) statistical density function that governs $Y_i^1$ with a positive location parameter shift by $\Delta$. The alternative $H_1$ therefore asserts that the predicted outcomes $\hat{Y}_i^1$, on average, are shifted by $\Delta > 0$ from the observed $Y_i^1$:
\begin{equation}
\mathbb{E}\left[\hat{Y}_i^1 - Y_i^1\right] = \Delta.
\end{equation}
If the alternative is assumed to be true, this would translate to the statement that the predicted counterfactual consumptions $\hat{Y}_i^1$, on average, are greater than the observed DR consumptions $Y_i^1$, which would imply a mean reduction of consumption by $\Delta$ during DR hours. The reasoning behind this is that we trained our estimators on standardized data $\left(X_i^0, Y_i^0\right)$, which results in consistent (unbiased?) estimators (BE MORE PRECISE HERE!!!!!!!!!). Predicting $\hat{Y}_i^1$ with the model which has been trained on non-DR data has the same structure as predicting $\hat{Y}_i^0$, since there is no a-priori knowledge of a DR event to predict $\hat{Y}_i^1$ (the covariates $X_i^0$ and $X_i^1$ both contain non-DR data only). The p-value with which $H_0$ is rejected provides a measure for the certainty of DR efficacy (= there is a reduction of consumption during DR events).


\subsection{Wilcoxon Signed Rank Test}
\label{sec:Wilcoxon}
The Wilcoxon signed rank test with paired samples $\left(\hat{Y}_i^1, Y_i^1\right)$ follows the intuition of the paired Student's $t$-test, with the specialty that the samples are not restricted to a normal distribution. The test places the pairwise differences into a single list which is then sorted in ascending order. Next, the rank of a data point is defined as its ordinal position in this sorted list. The test statistic $U$ involves the sum of the signed ranks, which can be approximated with a normal distribution
\begin{align}
U\sim\Ncal\left(\mu,\sigma\right),~ \mu = 0,~\sigma^2 = \frac{N(N+1)(2N+1)}{6},
\end{align}
where $N$ denotes the number of paired samples in $\left(\hat{Y}_i^1, Y_i^1\right)$.
In addition to the p-value, an estimate of the location parameter shift $\hat{\Delta}$ is provided by the test, which directly corresponds to the mean reduction of consumption during DR-events of user $i$, given the samples $\left(\hat{Y}_i^1, Y_i^1\right)$ \cite{Hettmansperger:2011aa, Lowry:1999aa}.
